Silo NLP's Participation at WAT2022

This paper provides the system description of "Silo NLP's" submission to the Workshop on Asian Translation (WAT2022). We have participated in the Indic Multimodal tasks (English->Hindi, English->Malayalam, and English->Bengali Multimodal Translation). For text-only translation, we trained Transformers from scratch and fine-tuned mBART-50 models. For multimodal translation, we used the same mBART architecture and extracted object tags from the images to use as visual features concatenated with the text sequence. Our submission tops many tasks including English->Hindi multimodal translation (evaluation test), English->Malayalam text-only and multimodal translation (evaluation test), English->Bengali multimodal translation (challenge test), and English->Bengali text-only translation (evaluation test).

==> mmt.tikz.tex <==
\tikzset{ shorten <>/.style={ shorten >=#1, shorten <=#1 } }

% some colors in hex:
%\definecolor{dblue}{HTML}{000492}
\definecolor{lgray}{HTML}{dddddd}

%\tikzstyle{vec} = [very thick, text width=17mm, minimum height=6mm, inner sep=0mm]
%\tikzstyle{vecgrid} = [shorten <>=.4mm]
%\tikzstyle{lstm} = [very thick, rounded corners, draw=green, fill=green!20,
%                    text width=15mm, minimum height=5mm, inner sep=0mm,
%                    text centered, font=\small, text=green]
\tikzstyle{hilight} = [draw=red, inner sep=0mm, very thick, rounded corners]

\tikzstyle{pil} = [draw, very thick, ->]
\tikzstyle{compute} = [draw, very thick, fill=lgray]
\tikzstyle{data} = [draw, thick, rounded corners, text width=4cm, text centered, font=\small]

\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[node distance = 2cm, on grid, auto]

\node[draw=black, inner sep=0] (img) {\includegraphics[width=2cm]{wat22_image.png}};
\node[below=0mm of img.south] (imglbl) {Image} {};

\node[compute, below=of img] (rcnn) {Faster R-CNN};

\node[data, below=of rcnn] (feats) {person,tennis racket,\\ potted plant,vase\strut};
\node[below=0mm of feats.south] (featslbl) {Object tags};

\node[data, right=5cm of img] (source) {A large pipe extending from the wall of the court.\strut};
\node[below=0mm of source.south] (sourcelbl) {Source text};

\coordinate (mid) at ($(img)!.5!(source)$);
\node[compute, below=6cm of mid] (concat) {Concatenate};

\node[data, below=of concat] (inp) {A large pipe \mbox{extending} from the wall of the court.\#\#person,tennis racket,potted plant,vase\strut};
\node[below=0mm of inp.south] (inplbl) {Input text};

\node[compute, below=2.5cm of inp] (mbart) {mBART-50};

\node[data, below=1.5cm of mbart] (out) {%\devanagari{कोर्ट की दीवार से निक्ली हुई एक बड़ी पाइप }};
\includegraphics[width=4cm]{hinditranslation.png}};
\node[below=0mm of out.south] (outlbl) {Translation};


\draw[pil] (imglbl) -- (rcnn);
\draw[pil] (rcnn) -- (feats);
\draw[pil] (featslbl) |- (concat);
\draw[pil] (sourcelbl) |- (concat);
\draw[pil] (concat) -- (inp);
\draw[pil] (inplbl) -- (mbart);
\draw[pil] (mbart) -- (out);

\end{tikzpicture}%
}

